Toward Scalable Fully Homomorphic Encryption Through Light Trusted Computing Assistance

It has been a long standing problem to securely outsource computation tasks to an untrusted party with integrity and confidentiality guarantees. While fully homomorphic encryption (FHE) is a promising technique that allows computations performed on the encrypted data, it suffers from a significant slow down to the computation. In this paper we propose a hybrid solution that uses the latest hardware Trusted Execution Environments (TEEs) to assist FHE by moving the bootstrapping step, which is one of the major obstacles in designing practical FHE schemes, to a secured SGX enclave. TEEFHE, the hybrid system we designed, makes it possible for homomorphic computations to be performed on smaller ciphertext and secret key, providing better performance and lower memory consumption. We make an effort to mitigate side channel leakages within SGX by making the memory access patterns totally independent from the secret information. The evaluation shows that TEEFHE effectively improves the software only FHE schemes in terms of both time and space.

==> tex/bio.tex <==
\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/wenhao.pdf}}]%
{Wenhao Wang} received the B.S. degree from Ocean University of China in 2009, and the Ph.D. degree from University of Chinese Academy of Sciences in 2015. He is an Associate Professor in Institute of Information Engineering, Chinese Academy of Sciences. His research interests include Cryptography, System Security, Cloud Security and Trusted Execution Technologies.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/yichen.pdf}}]%
{Yichen Jiang} recieved the M.S. degree of Computer Science from Syracuse University in 2017. In 2018 he is employed by UCSD department of biomedical informatics, and his research focuses on machine learning and secure computing. Currently he is a Ph.D. student at the University of Florida.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/qintao.pdf}}]%
{Qintao Shen} received his B.S. degree in the Henan Polytechnic University and M.S. degree in National University of Defense Technology (NUDT). He is currently pursuing a Ph.D. degree in the Institute of Information Engineering, Chinese Academy of Sciences. His research interests include software security, binary analysis, web security and Intel SGX.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/weihao.pdf}}]
{Weihao Huang} received his B.S. degree in the college of computer and software from Nanjing University of Posts and Telecommunications (NUPT) and M.S. degree in the college of cyberspace security from Beijing University of Posts and Telecommunications(BUPT). He is currently pursuing a Ph.D. degree in Institute of Information Engineering, Chinese Academy of Sciences. His research interests include automatic software security, program analysis and trusted computing based on Intel SGX.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/hao.pdf}}]%
{Hao Chen} obtained his Ph.D. degree in mathematics in 2016 from University of Washington. He is a researcher at Microsoft Research in Redmond working in the cryptography group. His research focuses on constructions, applications and cryptanalysis of fully homomorphic encryption (FHE) schemes.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/shuang.pdf}}]%
{Shuang Wang} (S’08–M’12) received the B.S. degree in applied physics and the M.S. degree in biomedical engineering from the Dalian University of Technology, China, and the Ph.D. degree in electrical and computer engineering from the University of Oklahoma, OK, USA, in 2012. He has worked as an assistant professor (2015 ~ 2018) and postdoc researcher (2012 ~ 2015) with the Department of Biomedical Informatics (DBMI), University of California, San Diego (UCSD), CA, USA. Currently, he is an assistant professor at the Assistant Professor of Computer Science, at the School of Informatics, Computing and Engineering. His research interests include machine learning, and healthcare data privacy/security. He has published more than 80+ journal/conference papers, 1 book and 3 book chapters. He was awarded a NGHRI K99/R00 career grant. Dr. Wang is a senior member of IEEE. Dr. Wang is a guest editor of Plos Genetics.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/XiaoFeng.pdf}}]%
{XiaoFeng Wang} is a James H. Rudy Professor of Computer Science and Engineering at Indiana University Bloomington. His research focuses on system security and data privacy with a specialization on security and privacy issues in mobile and cloud computing, and privacy issues in dissemination and computation of human genomic data.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/haixu.pdf}}]%
{Haixu Tang} is a professor of Computer Science and Engineering and adjunct professor of Biology at Indiana University Bloomington. He is a recipient of the NSF CAREER Award in 2007, and the outstanding junior faculty award in 2009. His research interests include computational mass spectrometry, privacy preserving techniques for analysis and dissemination of human genome data, mobile genetic elements and fragment assembly.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/kai.pdf}}]%
{Kai Chen} received the B.S. degree from Nanjing University in 2004, and the Ph.D. degree from University of Chinese Academy of Sciences in 2010. He is a Professor in Institute of Information Engineering, Chinese Academy of Sciences and also in the University of Chinese Academy of Sciences. His research interests include Software Security, Security Testing and AI security.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/kristin2.pdf}}]%
{Kristin Lauter} is a mathematician and cryptographer whose research areas are number theory, algebraic geometry, and applications to cryptography. She is particularly known for her work on homomorphic encryption, elliptic curve cryptography, and for introducing supersingular isogeny graphs as a hard problem into cryptography. She is a Principal Researcher and Research Manager of the Cryptography Group at Microsoft Research in Redmond, Washington. She served as President of the Association for Women in Mathematics from 2015 –2017. She is a Fellow of the American Mathematical Society, and the 2018-2020 Polya Lecturer for the Mathematical Association of America. She has published more than 100 papers and holds more than 50 patents.
\end{IEEEbiography}

\vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{files/dongdai.pdf}}]%
{Dongdai Lin} is a professor in Institute of Information Engineering, Chinese Academy of Sciences and in the University of Chinese Academy of Sciences. His research areas include Cryptology and Security Protocols.
\end{IEEEbiography}

==> tex/impl.tex <==
%\section{Implementation}
